On the relation between dynamic regret and closed-loop stability

In this work, we study the relations between bounded dynamic regret and the classical notion of asymptotic stability for the case of a priori unknown and time-varying cost functions. In particular, we show that bounded dynamic regret implies asymptotic stability of the optimal steady state for a constant cost function. For the case of an asymptotically stable closed loop, we first derive a necessary condition for achieving bounded dynamic regret. Then, given some additional assumptions on the system and the cost functions, we also provide a sufficient condition ensuring bounded dynamic regret. Our results are illustrated by examples.

==> figures/sketch.tex <==
\begin{tikzpicture}
	\clip(-1.25,-1.5) rectangle(7.25,2.5);
	\node[align = center, text width = 3cm] at (0,2) {\underline{time-invariant} \underline{cost functions}};
	\node[align = center, text width= 3cm] at (6,2) {\underline{time-varying} \underline{cost functions}};
	%\draw[dotted,thin] (3,7) -- (3,-3);
	\node[draw,ellipse,align=center,text width = 1.5cm] (stable) at (0,0) {asymptotic stability};
	\node[draw,ellipse,align=center, text width = 1.5cm] (regret) at (6,0) {bounded dynamic regret};
	
%	\draw[-{Stealth[length=3mm, width=2mm]}] (stable.20) -- node[fill=white,above,yshift=3ex] {Theorem~\ref{thm:stab_regret}} (regret.195);
%	\draw[-{Stealth[length=3mm, width=2mm]}] (regret.215) -- node[fill=white,below,xshift=5ex,yshift=-0.5ex] {Theorem~\ref{thm:regret_asymp_stab}} (stable.9);
	\draw[{Stealth[length=3mm, width=2mm]}-] (stable.350) to[out=310,in=230] node[fill=white,below,yshift=-.5ex,xshift=0ex] {Theorem~\ref{thm:regret_asymp_stab}} (regret.190);
	\draw[-{Stealth[length=3mm, width=2mm]}] (stable.10) to[out=50,in=135] node[fill=white,below,yshift=-1ex,xshift=0ex,align=center,text width = 10ex] {\textit{summable} $\mathcal{KL}$ bound} node[fill=white,above,yshift = 0.5ex,text width = 22ex,align = center] {Theorem~\ref{thm:stab_regret}, Proposition~\ref{prop:necessary_condition}} (regret.170);
\end{tikzpicture}
